Addressing Imbalance in Multi-Label Data via Label-Specific Distance-based Oversampling

The complex imbalanced label distribution poses a crucial challenge to multi-label classification, as most classifiers are biased towards the majority class and high-frequent labels. Oversampling is an efficient and flexible solution that augments instances to provide a more balanced training dataset for multi-label classifiers. Most existing oversampling methods create synthetic instances in a heuristic way that essentially relies on neighborhood information retrieved using Euclidean distance within the entire feature space. However, they fail to consider the varying semantic relevance of features to different labels, leading to label inconsistency among proximate neighbors and further introducing label confusion and overfitting to synthetic instances. To overcome the above issue, we propose a novel sampling approach called Label-Specific Distance-based Multi-Label Oversampling (LSDMLO) that creates more useful and well-labeled synthetic instances to address the imbalance in multi-label datasets. LSDMLO derives the label-specific distance to identify label-consistent neighbors based on the weighted pertinent feature space, which facilitates selecting seed instances that express more label correlations in boundary areas and generating synthetic instances aligned with the label distribution of original data. The comprehensive experiments verify that the proposed LSDMLO outperforms the state-of-the-art multi-label sampling approaches under various base classifiers.

==> tabel.tex <==

\begin{table}[!h]
\caption{Results of sampling methods with BR base learner}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
Datasets & Base & MLSMOTE\textsubscript{U} &  MLSMOTE\textsubscript{R} &  MLSOL & MLROS  & MLRUS & RHwRSMT & MLBOTE & LSDMLO  \\  \cmidrule(l){1-10} 
\multicolumn{10}{c} {Macro-F $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.5571(8) & 0.5589(6) & 0.5641(3) & 0.5626(4) & 0.5626(5) & 0.5574(7) & 0.3915(9) & \textbf{0.5692(1)} & 0.5671(2) \\
scene & 0.5850(6) & 0.5815(7) & 0.5805(8) & 0.5857(3) & 0.5855(4) & 0.5893(2) & 0.5684(9) & 0.5855(5) & \textbf{0.5940(1)} \\
yeast & 0.3883(6) & 0.3832(7) & 0.3885(5) & 0.3944(3) & 0.3832(8) & 0.3887(4) & 0.2741(9) & 0.3945(2) & \textbf{0.3961(1)} \\
Corel5k & 0.0591(7) & 0.0597(3) & 0.0596(4) & 0.0592(6) & 0.0601(2) & 0.0572(8) & 0.0417(9) & 0.0595(5) & \textbf{0.0607(1)} \\
rcv1subset1 & 0.2275(3) & 0.2222(8) & 0.2237(7) & 0.2243(5) & 0.2239(6) & 0.2248(4) & 0.1162(9) & 0.2284(2) & \textbf{0.2292(1)} \\
rcv1subset2 & 0.2011(4) & 0.1974(8) & 0.1983(7) & 0.2031(2) & 0.2016(3) & 0.1995(6) & 0.1084(9) & 0.2008(5) & \textbf{0.2033(1)} \\
rcv1subset3 & 0.2079(3) & 0.2011(8) & 0.2079(4) & \textbf{0.2087(1)} & 0.2055(6) & 0.2052(7) & 0.1128(9) & 0.2076(5) & 0.2084(2) \\
yahoo-Art & 0.2666(2) & 0.2635(7) & \textbf{0.2673(1)} & 0.2660(4) & 0.2639(6) & 0.2632(8) & 0.2200(9) & 0.2641(5) & 0.2663(3) \\
yahoo-Business & 0.2521(7) & 0.2565(6) & 0.2571(5) & 0.2595(2) & 0.2586(3) & 0.2505(8) & 0.2242(9) & 0.2586(4) & \textbf{0.2606(1)} \\\midrule
\textit{AveRank}& 5.11 & 6.67 & 4.89 & 3.33 & 4.78 & 6.00 & 9.00 & 3.78 & \textbf{1.44} \\\midrule
\multicolumn{10}{c} {Macro-AUC $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.6797(7) & 0.6828(3) & 0.6751(8) & 0.6832(2) & 0.6825(4) & 0.6806(6) & 0.6416(9) & 0.6825(5) & \textbf{0.6871(1)} \\
scene & 0.7472(7) & 0.7468(8) & 0.7458(9) & 0.7494(4) & 0.7473(5) & 0.7473(6) & 0.7521(2) & 0.7517(3) & \textbf{0.7542(1)} \\
yeast & 0.5631(4) & 0.5629(6) & 0.5627(7) & 0.5651(2) & 0.5597(8) & 0.5597(9) & 0.5638(3) & 0.5631(5) & \textbf{0.5669(1)} \\
Corel5k & 0.5210(7) & 0.5214(6) & 0.5216(4) & 0.5219(3) & 0.5215(5) & 0.5200(9) & 0.5210(8) & \textbf{0.5224(1)} & 0.5221(2) \\
rcv1subset1 & 0.6032(7) & 0.6049(3) & 0.6039(5) & 0.6081(2) & 0.6017(8) & 0.6033(6) & 0.5986(9) & 0.6044(4) & \textbf{0.6086(1)} \\
rcv1subset2 & 0.5914(6) & 0.5931(5) & 0.5937(4) & 0.5962(2) & 0.5907(7) & 0.5901(8) & 0.5891(9) & 0.5954(3) & \textbf{0.5981(1)} \\
rcv1subset3 & 0.5953(6) & 0.5972(4) & 0.5972(5) & \textbf{0.5997(1)} & 0.5947(9) & 0.5952(7) & 0.5952(8) &0.5983(3) & 0.5996(2) \\
yahoo-Art & 0.6159(6) & 0.6164(4) & 0.6167(3) & 0.6162(5) & 0.6139(9) & 0.6140(8) & 0.6159(7) & 0.6169(2) & \textbf{0.6173(1)} \\
yahoo-Business & 0.6278(8) & 0.6324(4) & 0.6310(7) & 0.6318(5) & 0.6313(6) & 0.6251(9) & \textbf{0.6344(1)} & 0.6333(3) & 0.6337(2) \\\midrule
\textit{AveRank}& 6.44 & 4.78 & 5.78 & 2.89 & 6.78 & 7.56 & 6.22 & 3.22 & \textbf{1.33} \\\midrule
\multicolumn{10}{c} {Macro-AUCPR $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.4574(6) & 0.4551(7) & 0.4584(5) & 0.4606(4) & 0.4625(2) & 0.4511(8) & 0.4290(9) & 0.4625(3) & \textbf{0.4648(1)} \\
scene & 0.4322(7) & 0.4271(8) & 0.4264(9) & 0.4331(4) & 0.4327(5) & 0.4395(3) & 0.4327(6) & 0.4414(2) & \textbf{0.4445(1)} \\
yeast & 0.3391(2) & 0.3368(7) & 0.3382(5) & 0.3386(4) & 0.3367(8) & 0.3389(3) & 0.3367(9) & 0.3370(6) & \textbf{0.3407(1)} \\
Corel5k & 0.0249(7) & 0.0246(8) & 0.0254(5) & 0.0255(2) & 0.0255(3) & 0.0251(6) & 0.0240(9) & 0.0255(4) & \textbf{0.0265(1)} \\
rcv1subset1 & 0.0973(8) & 0.0952(9) & 0.0982(4) & 0.0992(3) & 0.0978(6) & 0.0982(5) & 0.0976(7) & 0.0995(2) & \textbf{0.0996(1)} \\
rcv1subset2 & 0.0802(9) & 0.0817(4) & 0.0816(6) & 0.0826(3) & 0.0816(7) & 0.0817(5) & 0.0815(8) & 0.0827(2) & \textbf{0.0843(1)} \\
rcv1subset3 & 0.0871(3) & 0.0828(9) & 0.0867(6) & 0.0870(4) & 0.0862(7) & 0.0869(5) & 0.0862(8) & 0.0873(2) & \textbf{0.0903(1)} \\
yahoo-Art & 0.1316(2) & 0.1294(9) & 0.1307(5) & 0.1311(3) & 0.1306(6) & 0.1305(7) & 0.1304(8) & 0.1308(4) & \textbf{0.1385(1)} \\
yahoo-Business & 0.0993(8) & 0.1013(7) & 0.1029(3) & 0.1017(6) & 0.1025(4) & 0.0982(9) & 0.1025(5) & \textbf{0.1128(1)} & 0.1030(2) \\\midrule
\textit{AveRank} & 5.78 & 7.56 & 5.33 & 3.67 & 5.33 & 5.67 & 7.67 & 2.89 & \textbf{1.11} \\ \midrule
\multicolumn{10}{c} {Ranking Loss $\downarrow$} \\\cmidrule(l){1-10}
emotions & 0.5302(6) & 0.5341(8) & 0.5252(3) & 0.5299(4) & 0.5299(5) & 0.5330(7) & 0.6027(9) & \textbf{0.5225(1)}  & 0.5233(2) \\
scene & 0.4616(7) & 0.4622(8) & 0.4604(5) & 0.4605(6) & 0.4601(3) & 0.4624(9) & 0.4468(2) & 0.4601(4) & \textbf{4462(1)} \\
yeast & 0.5555(7) & 0.5523(4) & 0.5557(8) & 0.5705(9) & \textbf{0.5479(1)} & 0.5516(2) & 0.5534(6) & 0.5528(5) & 0.5519(3) \\
Corel5k & 0.8960(9) & 0.8758(3) & 0.8816(7) & 0.8747(2) & 0.8788(6) & 0.8783(4) & 0.8938(8) & 0.8786(5) & \textbf{0.8663(1)} \\
rcv1subset1 & 0.6392(7) & 0.6347(3) & 0.6380(6) & 0.6343(2) & 0.6392(8) & 0.6376(5) & 0.6470(9) & 0.6352(4) & \textbf{0.6300(1)} \\
rcv1subset2 & 0.6122(8) & 0.6090(5) & 0.6089(4) & \textbf{0.6032(1)} & 0.6118(7) & 0.6096(6) & 0.6171(9) & 0.6081(3) & 0.6054(2) \\
rcv1subset3 & 0.5972(7) & 0.5926(2) & 0.5961(6) & \textbf{0.5880(1)} & 0.5972(8) & 0.5956(5) & 0.6027(9) & 0.5953(4) & 0.5928(3) \\
yahoo-Art & \textbf{0.5117(1)} & 0.5168(7) & 0.5182(9) & 0.5143(3) & 0.5153(4) & 0.5154(6) & 0.5174(8) & 0.5153(5) & 0.5131(2) \\
yahoo-Business & 0.1852(5) & 0.1845(3) & 0.1854(7) & 0.1847(4) & 0.1853(6) & 0.1870(9) & 0.1856(8) & 0.1844(2) & \textbf{0.1837(1)} \\\midrule
 \textit{AveRank} & 6.33 & 4.78 & 6.11 & 3.56 & 5.33 & 5.89 & 7.56 & 3.67 & \textbf{1.78}
\\\bottomrule
\end{tabular}
}
\label{tab:BR}
\end{table}

\begin{table}[!h]
\caption{Results of sampling methods with MLkNN base learner}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
Datasets & Base & MLSMOTE\textsubscript{U} &  MLSMOTE\textsubscript{R} &  MLSOL & MLROS  & MLRUS & RHwRSMT & MLBOTE & LSDMLO  \\  \cmidrule(l){1-10} 
\multicolumn{10}{c} {Macro-F $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.4313(7) & 0.4325(5) & 0.4944(2) & 0.4885(3) & 0.4325(6) & 0.4216(8) & 0.2630(9) & \textbf{0.5295(1)} & 0.4787(4) \\
scene & 0.7348(3) & 0.7320(5) & 0.7433(2) & 0.7293(8) & 0.7320(6) & 0.7235(9) & 0.7298(7) & \textbf{0.7441(1)} & 0.7340(4) \\
yeast & 0.4006(8) & 0.4051(5) & 0.4131(3) & \textbf{0.4358(1)} & 0.4051(6) & 0.4035(7) & 0.2875(9) & 0.4122(4) & 0.4158(2) \\
Corel5k & 0.0344(5) & 0.0262(8) & 0.0344(6) & 0.0324(7) & \textbf{0.0375(1)} & 0.0349(3) & 0.0154(9) & 0.0351(2) & 0.0346(4) \\
rcv1subset1 & 0.1376(7) & 0.1673(5) & 0.1847(3) & \textbf{0.2242(1)} & 0.1673(6) & 0.1361(8) & 0.0973(9) & 0.1795(4) & 0.1937(2) \\
rcv1subset2 & 0.1375(7) & 0.1575(5) & 0.1745(3) & \textbf{0.2063(1)} & 0.1575(6) & 0.1353(8) & 0.0856(9) & 0.1612(4) & 0.1887(2) \\
rcv1subset3 & 0.1331(7) & 0.1580(6) & 0.1732(3) & \textbf{0.1988(1)} & 0.1582(5) & 0.1316(8) & 0.0801(9) & 0.1596(4) & 0.1954(2) \\
yahoo-Art & 0.1974(8) & 0.2217(3) & 0.2041(4) & 0.2222(2) & 0.1998(6) & 0.1990(7) & 0.1860(9) & 0.2039(5) & \textbf{0.2235(1)} \\
yahoo-Business & 0.1829(7) & 0.2052(3) & 0.1924(6) & 0.2217(2) & 0.1951(5) & 0.1821(8) & 0.1676(9) & 0.2000(4) & \textbf{0.2336(1)} \\\midrule
 \textit{AveRank} & 6.56 & 5.00 & 3.56 & 2.89 & 5.22 & 7.33 & 8.78 & 3.22 & \textbf{2.44} \\\midrule
 \multicolumn{10}{c} {Macro-AUC $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.7069(4) & 0.7064(6) & 0.7068(5) & 0.7026(8) & 0.7092(3) & 0.7064(7) & 0.6882(9) & 0.7097(2) & \textbf{0.7126(1)} \\
scene & 0.9254(6) & 0.9254(7) & 0.9258(4) & 0.9256(5) & \textbf{0.9261(1)} & 0.9254(8) & 0.9252(9) & 0.9259(3) & 0.9260(2) \\
yeast & 0.6704(4) & 0.6632(7) & 0.6698(5) & \textbf{0.6794(1)} & 0.6693(6) & 0.6632(8) & 0.6588(9) & 0.6739(2) & 0.6721(3) \\
Corel5k & 0.5484(7) & \textbf{0.5528(1)} & 0.5487(6) & 0.5494(5) & 0.5524(2) & 0.5479(8) & 0.5437(9) & 0.5513(3) & 0.5498(4) \\
rcv1subset1 & 0.7137(5) & 0.7056(7) & 0.7125(6) & 0.7301(2) & 0.7190(4) & 0.7056(8) & 0.7015(9) & 0.7247(3) & \textbf{0.7370(1)} \\
rcv1subset2 & 0.7021(5) & 0.6974(7) & 0.7013(6) & 0.7155(3) & 0.7115(4) & 0.6974(8) & 0.6933(9) & 0.7195(2) & \textbf{0.7232(1)} \\
rcv1subset3 & 0.7062(5) & 0.6985(7) & 0.7045(6) & 0.7171(3) & 0.7102(4) & 0.6985(8) & 0.6944(9) & 0.7203(2) & \textbf{0.7286(1)} \\
yahoo-Art & 0.6568(6) & 0.6557(8) & 0.6564(7) & 0.6601(4) & 0.6592(5) & 0.6557(9) & 0.6638(2) & \textbf{0.6683(1)} & 0.6632(3) \\
yahoo-Business & 0.6723(7) & 0.6764(5) & 0.6683(9) & \textbf{0.6823(1)} & 0.6744(6) & 0.6712(8) & 0.6770(4) & 0.6804(3) & 0.6806(2) \\
\midrule
 \textit{AveRank} & 5.44 & 6.11 & 6.00 & 3.56 & 3.89 & 8.00 & 7.67 & 2.33 & \textbf{2.00} \\\midrule
 \multicolumn{10}{c} {Macro-AUCPR $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.4931(5) & 0.4710(9) & 0.4921(6) & 0.4955(3) & 0.4912(7) & 0.4912(8) & 0.4940(4) & 0.4981(2) & \textbf{0.4989(1)} \\
scene & 0.7731(6) & 0.7776(3) & \textbf{0.7789(1)} & 0.7700(9) & 0.7739(5) & 0.7721(8) & 0.7731(7) & 0.7743(4) & 0.7787(2) \\
yeast & 0.4502(6) & 0.4444(8) & 0.4578(2) & 0.4535(5) & \textbf{0.4581(1)} & 0.4424(9) & 0.4502(7) & 0.4537(4) & 0.4551(3) \\
Corel5k & 0.0380(2) & 0.0359(8) & 0.0373(3) & 0.0367(6) & 0.0372(4) & 0.0366(7) & 0.0344(9) & 0.0369(5) & \textbf{0.0382(1)} \\
rcv1subset1 & 0.1645(8) & 0.1709(5) & 0.1741(4) & \textbf{0.1942(1)} & 0.1678(6) & 0.1671(7) & 0.1645(9) & 0.1774(3) & 0.1835(2) \\
rcv1subset2 & 0.1543(8) & 0.1546(7) & 0.1574(5) & \textbf{0.1768(1)} & 0.1575(4) & 0.1567(6) & 0.1542(9) & 0.1629(3) & 0.1673(2) \\
rcv1subset3 & 0.1529(7) & 0.1524(9) & 0.1578(4) & \textbf{0.1740(1)} & 0.1568(5) & 0.1561(6) & 0.1525(8) & 0.1626(3) & 0.1682(2) \\
yahoo-Art & 0.1972(6) & 0.2000(3) & 0.1932(7) & 0.2007(2) & 0.1975(5) & 0.1899(8) & 0.1899(9) & 0.1989(4) & \textbf{0.2041(1)} \\
yahoo-Business & 0.1560(8) & 0.1690(2) & 0.1641(5) & \textbf{0.1780(1)} & 0.1624(7) & 0.1628(6) & 0.1560(9) & 0.1675(4) & 0.1683(3) \\
\midrule
 \textit{AveRank}& 6.22 & 6.00 & 4.11 & 3.22 & 4.89 & 7.22 & 7.89 & 3.56 & \textbf{1.89} \\\midrule
 \multicolumn{10}{c} {Ranking Loss$\downarrow$} \\\cmidrule(l){1-10}
emotions & 0.2797(6) & \textbf{0.2709(1)} & 0.2798(8) & 0.2796(5) & 0.2766(2) & 0.2769(3) & 0.3160(9) & 0.2797(7) & 0.2772(4) \\
scene & 0.0874(3) & 0.0876(6) & 0.0883(8) & 0.0961(9) & 0.0871(2) & 0.0875(5) & 0.0877(7) & 0.0874(4) & \textbf{0.0859(1)} \\
yeast & 0.1869(4) & 0.1839(3) & 0.1869(5) & 0.1999(9) & \textbf{0.1795(1)} & 0.1873(7) & 0.1968(8) & 0.1869(6) & 0.1796(2) \\
Corel5k & 0.2048(6) & 0.2081(9) & 0.2073(8) & 0.2028(5) & 0.2004(3) & \textbf{0.1984(1)} & 0.2072(7) & 0.2021(4) & 0.1999(2) \\
rcv1subset1 & 0.1228(5) & 0.1282(9) & 0.1241(7) & \textbf{0.1195(1)} & 0.1196(2) & 0.1200(4) & 0.1258(8) & 0.1228(6) & 0.1197(3) \\
rcv1subset2 & 0.1155(6) & 0.1179(9) & 0.1138(5) & 0.1127(2) & \textbf{0.1123(1)} & 0.1129(4) & 0.1169(8) & 0.1155(7) & 0.1128(3) \\
rcv1subset3 & 0.1212(5) & 0.1253(9) & 0.1215(7) & \textbf{0.1162(1)} & 0.1174(3) & 0.1177(4) & 0.1237(8) & 0.1212(6) & 0.1173(2) \\
yahoo-Art & 0.1498(5) & 0.1524(7) & 0.1530(8) & 0.1490(4) & 0.1479(3) & \textbf{0.1472(1)} & 0.1539(9) & 0.1499(6) & 0.1476(2) \\
yahoo-Business & \textbf{0.1560(1)} & 0.1641(5) & 0.1683(7) & 0.1780(9) & 0.1675(6) & 0.1628(4) & 0.1690(8) & 0.1560(2) & 0.1624(3) \\
\midrule
 \textit{AveRank} & 4.56 & 6.44 & 7.00 & 5.00 & 2.56 & 3.67 & 8.00 & 5.33 & \textbf{2.44}
\\\bottomrule
\end{tabular}
}
\label{tab:MLkNN}
\end{table}

\begin{table}[!h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
Datasets & Base & MLSMOTE\textsubscript{U} &  MLSMOTE\textsubscript{R} &  MLSOL & MLROS  & MLRUS & RHwRSMT & MLBOTE & LSDMLO  \\  \cmidrule(l){1-10} 
\multicolumn{10}{c} {Macro-F $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.5549(5) & \textbf{0.5602(3)} & 0.5615(2) & 0.5583(4) & 0.5546(6) & 0.5540(8) & 0.4478(9) & 0.5546(7) & \textbf{0.5638(1)} \\
scene & 0.5865(4) & 0.5757(7) & 0.5737(8) & 0.5830(6) & 0.5887(2) & 0.5848(5) & 0.5611(9) & 0.5887(3) & \textbf{0.5903(1)} \\
yeast & 0.3826(7) & 0.3879(4) & 0.3858(6) & 0.3906(3) & 0.3826(8) & 0.3913(2) & 0.3036(9) & 0.3863(5) & \textbf{0.3977(1)} \\
Corel5k & 0.0509(8) & 0.0577(2) & 0.0555(7) & 0.0564(6) & 0.0577(3) & 0.0568(5) & 0.0412(9) & \textbf{0.0578(1)} & 0.0576(4) \\
rcv1subset1 & 0.2182(6) & 0.2152(8) & 0.2203(3) & 0.2217(2) & 0.2185(4) & 0.2173(7) & 0.1442(9) & 0.2185(5) & \textbf{0.2223(1)} \\
rcv1subset2 & 0.1967(7) & 0.1926(8) & 0.1991(5) & \textbf{0.2008(1)} & 0.2003(2) & 0.1985(6) & 0.1362(9) & 0.1996(4) & 0.2002(3) \\
rcv1subset3 & 0.2017(6) & 0.1972(8) & 0.2022(5) & 0.2052(2) & 0.2046(3) & 0.2009(7) & 0.1345(9) & 0.2032(4) & \textbf{0.2054(1)} \\
yahoo-Art & 0.2547(6) & 0.2506(8) & 0.2555(5) & \textbf{0.2572(1)} & 0.2547(7) & 0.2559(4) & 0.2320(9) & 0.2562(3) & 0.2563(2) \\
yahoo-Business & 0.2434(7) & 0.2444(6) & 0.2490(5) & 0.2493(4) & 0.2502(2) & 0.2428(8) & 0.2331(9) & 0.2502(3) & \textbf{0.2527(1)} \\
\midrule
\textit{AveRank} & 6.22 & 6.00 & 5.11 & 3.22 & 4.11 & 5.78 & 9.00 & 3.89 & \textbf{1.67} \\\midrule
\multicolumn{10}{c} {Macro-AUC $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.6783(4) & 0.6772(7) & 0.6817(2) & 0.6793(3) & 0.6776(5) & 0.6771(8) & 0.6370(9) & 0.6776(6) & \textbf{0.6853(1)} \\
scene & 0.7485(4) & 0.7422(7) & 0.7402(9) & 0.7473(6) & 0.7489(2) & 0.7479(5) & 0.7418(8) & 0.7489(3) & \textbf{0.7501(1)} \\
yeast & 0.5618(3) & 0.5567(8) & 0.5603(4) & 0.5590(5) & 0.5589(6) & \textbf{0.5633(1)} & 0.5468(9) & 0.5589(7) & 0.5625(2) \\
Corel5k & 0.5207(5) & 0.5175(8) & 0.5202(7) & 0.5211(2) & 0.5208(4) & 0.5204(6) & 0.5144(9) & \textbf{0.5217(1)} & 0.5209(3) \\
rcv1subset1 & 0.5994(7) & 0.5995(5) & 0.6026(4) & 0.6028(3) & 0.5995(6) & 0.5988(8) & 0.5738(9) & 0.6031(2) & \textbf{0.6042(1)} \\
rcv1subset2 & 0.5909(8) & 0.5914(6) & 0.5916(5) & 0.5924(3) & 0.5919(4) & 0.5911(7) & 0.5664(9) & 0.5933(2) & \textbf{0.5972(1)} \\
rcv1subset3 & 0.5935(7) & 0.5935(8) & 0.5966(2) & 0.5959(5) & 0.5965(4) & 0.5950(6) & 0.5691(9) & 0.5966(3) & \textbf{0.5990(1)} \\
yahoo-Art & 0.6112(4) & 0.6098(6) & 0.6124(2) & 0.6105(5) & 0.6098(7) & 0.6096(8) & 0.6036(9) & 0.6116(3) & \textbf{0.6125(1)} \\
yahoo-Business & 0.6263(7) & 0.6289(6) & 0.6296(2) & \textbf{0.6317(1)} & 0.6291(4) & 0.6235(8) & 0.6163(9) & 0.6291(5) & 0.6293(3) \\\midrule
\textit{AveRank} & 5.44 & 6.78 & 4.11 & 3.67 & 4.67 & 6.33 & 8.89 & 3.56 & \textbf{1.56} \\\midrule
\multicolumn{10}{c} {Macro-AUCPR $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.4570(3) & 0.4514(8) & 0.4522(7) & 0.4577(2) & 0.4570(4) & 0.4567(6) & 0.4216(9) & 0.4570(5) & \textbf{0.4606(1)} \\
scene & 0.4339(4) & 0.4235(8) & 0.4208(9) & 0.4304(6) & 0.4364(2) & 0.4334(5) & 0.4290(7) & 0.4364(3) & \textbf{0.4382(1)} \\
yeast & 0.3354(6) & 0.3345(7) & 0.3366(4) & \textbf{0.3391(1)} & 0.3372(3) & 0.3344(8) & 0.3318(9) & 0.3357(5) & 0.3377(2) \\
Corel5k & 0.0234(8) & 0.0238(7) & 0.0240(6) & 0.0249(3) & \textbf{0.0252(1)} & 0.0245(5) & 0.0226(9) & 0.0249(4) & 0.0252(2) \\
rcv1subset1 & 0.0945(6) & 0.0920(8) & 0.0946(4) & 0.0954(3) & 0.0946(5) & 0.0942(7) & 0.0824(9) & 0.0958(2) & \textbf{0.0963(1)} \\
rcv1subset2 & 0.0800(6) & 0.0775(8) & 0.0798(7) & 0.0809(2) & 0.0807(4) & 0.0804(5) & 0.0713(9) & 0.0808(3) & \textbf{0.0814(1)} \\
rcv1subset3 & 0.0829(5) & 0.0800(8) & 0.0828(6) & 0.0844(3) & 0.0841(4) & 0.0827(7) & 0.0738(9) & 0.0846(2) & \textbf{0.0848(1)} \\
yahoo-Art & 0.1248(6) & 0.1230(9) & 0.1250(5) & 0.1255(2) & 0.1248(7) & 0.1251(4) & 0.1237(8) & 0.1252(3) & \textbf{0.1282(1)} \\
yahoo-Business & 0.0958(8) & 0.0961(7) & 0.0986(2) & 0.0977(6) & 0.0983(4) & 0.0950(9) & 0.0986(3) & 0.0983(5) & \textbf{0.0992(1)} \\
\midrule
\textit{AveRank}  & 5.78 & 7.78 & 5.56 & 3.11 & 3.78 & 6.22 & 8.00 & 3.56 & \textbf{1.22} \\\midrule
\multicolumn{10}{c} {Ranking Loss $\downarrow$} \\\cmidrule(l){1-10}
emotions & 0.5229(6) & 0.5299(8) & \textbf{0.5087(1)} & 0.5174(3) & 0.5215(4) & 0.5251(7) & 0.6086(9) & 0.5215(5) & 0.5089(2) \\
scene & 0.4369(4) & 0.4503(6) & 0.4542(8) & 0.4523(7) & 0.4362(2) & 0.4484(5) & 0.4571(9) & 0.4362(3) & \textbf{0.4346(1)} \\
yeast & 0.5517(2) & 0.5594(7) & 0.5579(5) & 0.5705(8) & 0.5586(6) & \textbf{0.5474(1)} & 0.6513(9) & 0.5552(3) & 0.5552(4) \\
Corel5k & 0.8783(5) & 0.8890(8) & 0.8826(7) & 0.8763(3) & 0.8790(6) & 0.8776(4) & 0.9205(9) & \textbf{0.8638(1)} & 0.8760(2) \\
rcv1subset1 & 0.6416(5) & 0.6453(7) & 0.6414(4) & \textbf{0.6313(1)} & 0.6453(8) & 0.6442(6) & 0.7232(9) & 0.6372(2) & 0.6404(3) \\
rcv1subset2 & 0.6100(4) & 0.6154(8) & 0.6120(5) & \textbf{0.6032(1)} & 0.6140(7) & 0.6121(6) & 0.6962(9) & 0.6082(2) & 0.6098(3) \\
rcv1subset3 & 0.5950(3) & 0.5982(8) & 0.5963(5) & \textbf{0.5852(1)} & 0.5973(7) & 0.5971(6) & 0.6845(9) & 0.5946(2) & 0.5957(4) \\
yahoo-Art & 0.5093(4) & 0.5112(7) & 0.5133(8) & 0.5098(5) & 0.5092(2) & 0.5101(6) & 0.5507(9) & 0.5092(3) & \textbf{0.5085(1)} \\
yahoo-Business & 0.1868(5) & 0.1873(6) & 0.1876(7) & 0.1863(2) & 0.1864(3) & 0.1877(8) & 0.1934(9) & 0.1864(4) & \textbf{0.1856(1)}\\\midrule 
 \textit{AveRank}  & 4.22 & 7.22 & 5.56 & 3.44 & 5.00 & 5.44 & 9.00 & 2.78 & \textbf{2.33}
\\\bottomrule
\end{tabular}
}
\caption{Results of sampling methods with CC base learner}
\label{tab:CC}
\end{table}

\begin{table}[!h]
\caption{Results of sampling methods with RAkEL base learner}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
Datasets & Base & MLSMOTE\textsubscript{U} &  MLSMOTE\textsubscript{R} &  MLSOL & MLROS  & MLRUS & RHwRSMT & MLBOTE & LSDMLO  \\  \cmidrule(l){1-10} 
\multicolumn{10}{c} {Macro-F $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.5458(8) & \textbf{0.5614(1)} & 0.5571(3) & 0.5549(5) & 0.5568(4) & 0.5465(7) & 0.4328(9) & 0.5546(6) & 0.5579(2) \\
scene & 0.5807(7) & 0.5797(8) & 0.5812(6) & 0.5821(5) & 0.5834(3) & 0.5842(2) & 0.5699(9) & 0.5828(4) & \textbf{0.5866(1)} \\
yeast & 0.3803(7) & 0.3823(6) & 0.3832(5) & 0.3925(2) & 0.3855(3) & 0.3789(8) & 0.3034(9) & 0.3841(4) & \textbf{0.3926(1)} \\
Corel5k & 0.0566(7) & 0.0581(5) & 0.0559(8) & 0.0603(2) & 0.0585(4) & 0.0575(6) & 0.0411(9) & 0.0589(3) & \textbf{0.0604(1)} \\
rcv1subset1 & 0.2139(6) & 0.2138(7) & 0.2136(8) & 0.2174(2) & 0.2159(4) & 0.2155(5) & 0.1236(9) & 0.2165(3) & \textbf{0.2206(1)} \\
rcv1subset2 & 0.1924(7) & 0.1905(8) & 0.1975(4) & 0.1929(6) & 0.1987(2) & 0.1947(5) & 0.1142(9) & 0.1983(3) & \textbf{0.1999(1)} \\
rcv1subset3 & 0.2009(6) & 0.1968(8) & 0.2032(4) & 0.2044(2) & 0.2013(5) & 0.1999(7) & 0.1166(9) & 0.2044(3) & \textbf{0.2048(1)} \\
yahoo-Art & 0.2669(6) & 0.2636(8) & 0.2646(7) & 0.2684(2) & 0.2681(3) & 0.2680(4) & 0.2207(9) & 0.2678(5) & \textbf{0.2702(1)} \\
yahoo-Business & 0.2578(7) & 0.2629(4) & 0.2603(5) & 0.2586(6) & \textbf{0.2686(1)} & 0.2503(8) & 0.2254(9) & 0.2640(3) & 0.2646(2) \\
\midrule
\textit{AveRank} & 6.78 & 6.11 & 5.56 & 3.56 & 3.22 & 5.78 & 9.00 & 3.78 & \textbf{1.22} \\\midrule
\multicolumn{10}{c} {Macro-AUC $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.6707(6) & 0.6771(2) & 0.6767(3) & 0.6691(8) & 0.6764(4) & 0.6707(7) & 0.6430(9) & 0.6760(5) & \textbf{0.6785(1)} \\
scene & 0.7430(9) & 0.7446(7) & 0.7466(4) & 0.7433(8) & 0.7449(6) & 0.7469(3) & \textbf{0.7481(1)} & 0.7450(5) & 0.7478(2) \\
yeast & 0.5583(7) & 0.5584(6) & 0.5585(5) & 0.5598(2) & \textbf{0.5611(1)} & 0.5574(8) & 0.5561(9) & 0.5588(4) & 0.5592(3) \\
Corel5k & 0.5197(9) & 0.5214(4) & 0.5208(5) & 0.5224(2) & 0.5207(6) & 0.5201(8) & 0.5202(7) & 0.5219(3) & \textbf{0.5237(1)} \\
rcv1subset1 & 0.5967(8) & 0.5972(6) & 0.5990(4) & 0.6010(2) & 0.5977(5) & 0.5969(7) & 0.5965(9) & 0.6007(3) & \textbf{0.6023(1)} \\
rcv1subset2 & 0.5868(9) & 0.5891(5) & 0.5910(3) & \textbf{0.5941(1)} & 0.5881(6) & 0.5876(7) & 0.5872(8) & 0.5903(4) & 0.5916(2) \\
rcv1subset3 & 0.5920(7) & 0.5935(6) & 0.5946(3) & \textbf{0.5954(1)} & 0.5937(5) & 0.5914(8) & 0.5891(9) & 0.5945(4) & 0.5951(2) \\
yahoo-Art & 0.6119(9) & 0.6133(6) & 0.6129(7) & \textbf{0.6142(1)} & 0.6135(3) & 0.6127(8) & 0.6134(5) & 0.6135(4) & 0.6141(2) \\
yahoo-Business & 0.6259(8) & 0.6294(5) & 0.6292(7) & 0.6293(6) & 0.6315(2) & 0.6222(9) & 0.6298(4) & 0.6303(3) & \textbf{0.6326(1)} \\
\midrule
\textit{AveRank}& 8.00 & 5.22 & 4.56 & 3.44 & 4.22 & 7.22 & 6.78 & 3.89 & \textbf{1.67} \\\midrule
\multicolumn{10}{c} {Macro-AUCPR $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.4468(7) & 0.4330(9) & 0.4514(4) & \textbf{0.4581(1)} & 0.4505(5) & 0.4433(8) & 0.4475(6) & 0.4554(2) & 0.4551(3) \\
scene & 0.4274(7) & 0.4289(6) & 0.4308(4) & 0.4318(3) & 0.4304(5) & 0.4263(9) & 0.4273(8) & 0.4336(2) & \textbf{0.4409(1)} \\
yeast & 0.3364(2) & 0.3361(5) & 0.3357(8) & \textbf{0.3370(1)} & 0.3362(3) & 0.3359(6) & 0.3346(9) & 0.3358(7) & 0.3362(4) \\
Corel5k & 0.0248(7) & 0.0240(9) & 0.0252(4) & 0.0252(5) & 0.0256(2) & 0.0251(6) & 0.0245(8) & 0.0256(3) & \textbf{0.0257(1)} \\
rcv1subset1 & 0.0934(7) & 0.0927(8) & 0.0952(3) & 0.0946(4) & 0.0938(6) & 0.0945(5) & 0.0911(9) & \textbf{0.0967(1)} & 0.0962(2) \\
rcv1subset2 & 0.0789(8) & 0.0795(6) & 0.0791(7) & 0.0814(3) & 0.0808(4) & 0.0798(5) & 0.0768(9) & 0.0820(2) & \textbf{0.0830(1)} \\
rcv1subset3 & \textbf{0.0859(1)} & 0.0827(8) & 0.0848(4) & 0.0839(6) & 0.0847(5) & 0.0839(7) & 0.0815(9) & 0.0854(3) & 0.0859(2) \\
yahoo-Art & 0.1314(7) & 0.1326(5) & 0.1314(8) & 0.1334(3) & 0.1334(4) & 0.1323(6) & 0.1298(9) & 0.1338(2) & \textbf{0.1388(1)} \\
yahoo-Business & 0.1039(7) & 0.1073(3) & 0.1055(6) & 0.1082(2) & 0.1022(8) & 0.1002(9) & 0.1059(5) & 0.1066(4) & \textbf{0.1133(1)} \\
\midrule
\textit{AveRank} & 5.89 & 6.56 & 5.33 & 3.11 & 4.67 & 6.78 & 8.00 & 2.89 & \textbf{1.78} \\\midrule
\multicolumn{10}{c} {Ranking Loss $\downarrow$} \\\cmidrule(l){1-10}
emotions & 0.5375(8) & 0.5272(5) & 0.5202(2) & 0.5245(4) & 0.5313(7) & 0.5306(6) & 0.6077(9) & \textbf{0.5180(1)} & 0.5212(3) \\
scene & 0.4489(5) & 0.4519(7) & 0.4423(3) & 0.4467(4) & 0.4690(9) & 0.4534(8) & \textbf{0.4376(1)} & 0.4513(6) & 0.4381(2) \\
yeast & 0.5542(3) & 0.5580(5) & 0.5599(6) & \textbf{0.5534(1)} & 0.5738(9) & 0.5556(4) & 0.5616(8) & 0.5610(7) & 0.5537(2) \\
Corel5k & 0.8815(6) & 0.8983(9) & 0.8841(7) & \textbf{0.8684(1)} & 0.8750(2) & 0.8809(5) & 0.8965(8) & 0.8804(4) & 0.8772(3) \\
rcv1subset1 & 0.6433(5) & 0.6449(7) & 0.6454(8) & \textbf{0.6371(1)} & 0.6403(3) & 0.6437(6) & 0.6510(9) & 0.6432(4) & 0.6377(2) \\
rcv1subset2 & 0.6137(6) & 0.6153(7) & 0.6166(8) & 0.6102(3) & \textbf{0.6066(1)} & 0.6131(5) & 0.6201(9) & 0.6115(4) & 0.6097(2) \\
rcv1subset3 & 0.5973(5) & 0.5982(7) & 0.5997(8) & 0.5925(2) & 0.5956(4) & 0.5976(6) & 0.6081(9) & 0.5936(3) & \textbf{0.5917(1)} \\
yahoo-Art & 0.5135(4) & 0.5154(5) & 0.5186(8) & 0.5160(7) & 0.5154(6) & 0.5134(3) & 0.5237(9) & 0.5127(2) & \textbf{0.5114(1)} \\
yahoo-Business & 0.1865(7) & \textbf{0.1837(1)} & 0.1856(4) & 0.1859(5) & 0.1865(8) & 0.1873(9) & 0.1862(6) & 0.1845(2) & 0.1848(3) \\
\midrule
 \textit{AveRank} & 5.44 & 5.89 & 6.00 & 3.11 & 5.44 & 5.78 & 7.56 & 3.67 & \textbf{2.11}
\\\bottomrule
\end{tabular}
}
\label{tab:RAkEL}
\end{table}

\begin{table}[!h]
\caption{Results of sampling methods with COCOA base learner}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
Datasets & Base & MLSMOTE\textsubscript{U} &  MLSMOTE\textsubscript{R} &  MLSOL & MLROS  & MLRUS & RHwRSMT & MLBOTE & LSDMLO  \\  \cmidrule(l){1-10} 
\multicolumn{10}{c} {Macro-F $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.6239(8) & 0.6277(5) & 0.6344(3) & 0.6306(4) & 0.6277(6) & 0.6267(7) & 0.5773(9) & 0.6360(2) & \textbf{0.6361(1)} \\
scene & 0.7214(2) & 0.7194(8) & 0.7200(6) & 0.7207(4) & 0.7203(5) & 0.7197(7) & 0.7173(9) & 0.7209(3) & \textbf{0.7216(1)} \\
yeast & 0.4565(9) & 0.4689(5) & 0.4714(3) & 0.4689(6) & 0.4679(7) & 0.4711(4) & 0.4679(8) & 0.4719(2) & \textbf{0.4721(1)} \\
Corel5k & 0.0957(4) & 0.0955(6) & 0.0942(7) & 0.0962(3) & \textbf{0.0976(1)} & 0.0921(8) & 0.0875(9) & 0.0957(5) & 0.0973(2) \\
rcv1subset1 & 0.2969(8) & 0.3257(3) & 0.3257(4) & 0.3246(5) & 0.3263(2) & 0.2960(9) & 0.3002(7) & 0.3229(6) & \textbf{0.3346(1)} \\
rcv1subset2 & 0.2790(9) & 0.3058(6) & 0.3099(2) & 0.3088(4) & 0.3090(3) & 0.2797(8) & 0.2879(7) & 0.3083(5) & \textbf{0.3103(1)} \\
rcv1subset3 & 0.2806(8) & 0.3071(5) & 0.3081(4) & 0.3089(3) & \textbf{0.3140(1)} & 0.2799(9) & 0.2965(7) & 0.2999(6) & 0.3103(2) \\
yahoo-Art & 0.3347(7) & 0.3360(6) & 0.3366(5) & \textbf{0.3387(1)} & 0.3374(3) & 0.3217(9) & 0.3218(8) & 0.3372(4) & 0.3376(2) \\
yahoo-Business & 0.3396(4) & 0.3377(6) & 0.3393(5) & 0.3458(2) & 0.3376(7) & 0.3321(9) & 0.3376(8) & 0.3415(3) & \textbf{0.3465(1)} \\
\midrule
 \textit{AveRank} & 6.56 & 5.56 & 4.33 & 3.56 & 3.89 & 7.78 & 8.00 & 4.00 & \textbf{1.33} \\ \midrule
 \multicolumn{10}{c}{Macro-AUC $\uparrow$} \\\cmidrule(l){1-10} 
emotions & 0.7928(3) & 0.7912(7) & 0.7920(6) & 0.7923(5) & 0.7928(4) & 0.7910(8) & 0.7749(9) & 0.7932(2) & \textbf{0.7946(1)} \\
scene & \textbf{0.9251(1)} & 0.9233(8) & 0.9245(4) & 0.9238(7) & 0.9245(5) & 0.9246(3) & 0.9231(9) & 0.9245(6) & 0.9248(2) \\
yeast & 0.6743(6) & 0.6756(5) & 0.6778(3) & \textbf{0.6802(1)} & 0.6743(7) & 0.6741(8) & 0.6733(9) & 0.6758(4) & 0.6801(2) \\
Corel5k & \textbf{0.6996(1)} & 0.6915(9) & 0.6957(7) & 0.6991(3) & 0.6987(4) & 0.6977(6) & 0.6949(8) & 0.6986(5) & 0.6993(2) \\
rcv1subset1 & 0.8758(7) & 0.8947(3) & 0.8917(4) & 0.8909(5) & 0.8950(2) & 0.8749(8) & 0.8683(9) & 0.8881(6) & \textbf{0.8962(1)} \\
rcv1subset2 & 0.8803(7) & 0.8957(3) & 0.8922(5) & 0.8871(6) & 0.8959(2) & 0.8792(8) & 0.8754(9) & 0.8952(4) & \textbf{0.8976(1)} \\
rcv1subset3 & 0.9013(8) & 0.9014(7) & 0.9100(2) & 0.9051(5) & 0.9077(3) & 0.9005(9) & 0.9030(6) & 0.9055(4) & \textbf{0.9102(1)} \\
yahoo-Art & 0.7494(3) & 0.7445(8) & 0.7478(6) & 0.7495(2) & 0.7481(5) & 0.7462(7) & 0.7336(9) & 0.7482(4) & \textbf{0.7502(1)} \\
yahoo-Business & 0.7691(7) & 0.7704(4) & 0.7699(5) & \textbf{0.7724(1)} & 0.7699(6) & 0.7680(8) & 0.7575(9) & 0.7710(2) & 0.7706(3) \\
\midrule
 \textit{AveRank} & 4.78 & 6.00 & 4.67 & 3.89 & 4.22 & 7.22 & 8.56 & 4.11 & \textbf{1.56} \\\midrule
 \multicolumn{10}{c}{Macro-AUCPR $\uparrow$} \\\cmidrule(l){1-10} 
emotions & 0.6408(5) & 0.6335(8) & 0.6375(7) & 0.6400(6) & \textbf{0.6460(1)} & 0.6411(4) & 0.6166(9) & 0.6460(2) & 0.6423(3) \\
scene & 0.7755(4) & 0.7723(8) & 0.7741(7) & 0.7749(6) & 0.7755(5) & 0.7759(3) & 0.7699(9) & 0.7760(2) & \textbf{0.7770(1)} \\
yeast & 0.4592(5) & 0.4549(9) & 0.4584(7) & 0.4601(4) & 0.4592(6) & 0.4624(2) & 0.4579(8) & 0.4604(3) & \textbf{0.4627(1)} \\
Corel5k & 0.0850(6) & 0.0803(9) & 0.0848(7) & 0.0851(5) & 0.0856(4) & 0.0857(3) & 0.0839(8) & 0.0858(2) & \textbf{0.0860(1)} \\
rcv1subset1 & 0.2903(7) & 0.2990(5) & 0.2979(6) & 0.3003(2) & 0.2997(3) & 0.2893(8) & 0.2794(9) & 0.2997(4) & \textbf{0.3005(1)} \\
rcv1subset2 & 0.2707(7) & 0.2777(6) & 0.2782(5) & 0.2799(2) & 0.2797(3) & 0.2695(8) & 0.2670(9) & 0.2791(4) & \textbf{0.2846(1)} \\
rcv1subset3 & 0.2723(8) & 0.2825(5) & 0.2802(6) & 0.2849(2) & 0.2843(3) & 0.2710(9) & 0.2767(7) & 0.2834(4) & \textbf{0.2899(1)} \\
yahoo-Art & 0.2768(2) & 0.2659(9) & 0.2740(7) & \textbf{0.2786(1)} & 0.2747(5) & 0.2763(4) & 0.2685(8) & 0.2747(6) & 0.2766(3) \\
yahoo-Business & 0.2647(3) & 0.2567(9) & 0.2638(4) & \textbf{0.2707(1)} & 0.2632(6) & 0.2625(8) & 0.2627(7) & 0.2636(5) & 0.2703(2) \\
\midrule
 \textit{AveRank} & 5.22 & 7.56 & 6.22 & 3.22 & 4.00 & 5.44 & 8.22 & 3.56 & \textbf{1.56} \\\midrule
 \multicolumn{10}{c}{Ranking Loss $\downarrow$} \\\cmidrule(l){1-10} 
emotions & 0.2016(7) & \textbf{0.1995(1)} & 0.2028(8) & 0.2013(6) & 0.2004(2) & 0.2007(5) & 0.2357(9) & 0.2004(3) & 0.2006(4) \\
scene & 0.0833(4) & 0.0858(9) & 0.0844(6) & \textbf{0.0814(1)} & 0.0837(5) & 0.0849(8) & 0.0846(7) & 0.0827(3) & 0.0822(2) \\
yeast & 0.1781(7) & 0.1738(3) & 0.1751(4) & 0.1830(9) & 0.1775(5) & 0.1790(8) & 0.1775(6) & 0.1730(2) & \textbf{0.1712(1)} \\
Corel5k & 0.1672(8) & 0.1676(9) & 0.1671(7) & 0.1662(6) & 0.1661(4) & 0.1654(2) & 0.1661(5) &  \textbf{0.1651(1)} & 0.1654(3) \\
rcv1subset1 & 0.0747(8) & 0.0685(6) & 0.0687(7) & 0.0682(5) & 0.0671(2) & 0.0752(9) & 0.0678(4) & 0.0674(3) & \textbf{0.0605(1)} \\
rcv1subset2 & 0.0708(8) & 0.0654(6) & 0.0654(7) & 0.0632(2) & 0.0642(3) & 0.0712(9) & 0.0647(5) & 0.0642(4) & \textbf{0.0601(1)} \\
rcv1subset3 & 0.0721(9) & 0.0670(5) & 0.0659(2) & 0.0668(4) & 0.0667(3) & 0.0676(7) & 0.0714(8) & 0.0672(6) & \textbf{0.0648(1)} \\
yahoo-Art & 0.1300(9) & 0.1291(6) & 0.1296(8) & 0.1288(3) & 0.1287(2) & 0.1292(7) & \textbf{0.1202(1)} & 0.1288(4) & 0.1289(5) \\
yahoo-Business & 0.0407(3) & 0.0412(9) & 0.0410(8) & 0.0408(6) & 0.0407(4) & 0.0409(7) & \textbf{0.0352(1)} & 0.0407(5) & 0.0399(2) \\
\midrule
 \textit{AveRank} & 7.00 & 6.00 & 6.33 & 4.67 & 3.33 & 6.89 & 5.11 & 3.44 & \textbf{2.22}
\\\bottomrule
\end{tabular}
}
\label{tab:COCOA}
\end{table}

\begin{table}[!h]
\caption{Results of sampling methods with C2AE deep learner}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
Datasets & Base & MLSMOTE\textsubscript{U} &  MLSMOTE\textsubscript{R} &  MLSOL & MLROS  & MLRUS & RHwRSMT & MLBOTE & LSDMLO  \\  \cmidrule(l){1-10} 
\multicolumn{10}{c} {Macro-F $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.5373(8) & \textbf{0.6099(1)} & 0.5994(2) & 0.5962(3) & 0.5651(7) & 0.5938(4) & 0.5193(9) & 0.5938(5) & 0.5908(6) \\
scene & 0.7884(4) & 0.7749(9) & 0.7792(8) & 0.7868(5) & 0.7823(6) & 0.7808(7) & 0.7936(2) & 0.7898(3) & \textbf{0.7971(1)} \\
yeast & 0.4111(8) & 0.4251(4) & 0.4186(5) & 0.4146(6) & 0.4320(3) & 0.4124(7) & 0.4084(9) & 0.4424(2) & \textbf{0.4672(1)} \\
Corel5k & 0.1281(7) & 0.1322(5) & 0.1201(8) & \textbf{0.1362(1)} & 0.1294(6)  & 0.1333(4)& 0.1077(9) & 0.1362(2) & 0.1340(3) \\
rcv1subset1 & 0.3205(7) & 0.3160(8) & 0.3315(4) & 0.3225(6) & 0.3314(5) & 0.3329(2) & 0.2068(9) & 0.3329(3) & \textbf{0.3388(1)} \\
rcv1subset2 & 0.2640(9) & 0.2971(7) & 0.3264(5) & 0.3285(4) & 0.3322(2) & 0.3191(6) & 0.2908(8) & 0.3291(3) & \textbf{0.3346(1)} \\
rcv1subset3 & 0.2301(9) & 0.2551(6) & 0.2657(4) & \textbf{0.2924(1)} & 0.2673(3) & 0.2469(7) & 0.2450(8) & 0.2569(5) & 0.2822(2) \\
yahoo-Art & 0.3417(8) & 0.3519(5) & 0.3594(2) & 0.3563(3) & 0.3523(4) & 0.3425(6) & 0.3253(9) & 0.3425(7) & \textbf{0.3646(1)} \\
yahoo-Business & 0.4124(9) & 0.4266(8) & 0.4331(2) & 0.4283(4) & 0.4276(5) & 0.4273(6) & 0.4252(7) & 0.4313(3) & \textbf{0.4337(1)} \\
\midrule
\textit{AveRank}  & 7.67 & 5.89 & 4.44 & 4.22 & 4.56 & 4.89 & 7.78 & 3.67 & \textbf{1.89} \\\midrule
\multicolumn{10}{c} {Macro-AUC $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.8208(9) & 0.8219(8) & 0.8265(5) & 0.8258(6) & 0.8288(2) & 0.8278(4) & 0.8239(7) & 0.8286(3) & \textbf{0.8316(1)} \\
scene & 0.9462(9) & 0.9492(6) & 0.9490(7) & \textbf{0.9547(1)} & 0.9508(4) & 0.9484(8) & 0.9530(3) & 0.9502(5) & 0.9542(2) \\
yeast & 0.7005(7) & 0.7004(8) & 0.7009(6) & 0.7088(2) & 0.7063(3) & 0.7022(5) & 0.6796(9) & 0.7062(4) & \textbf{0.7370(1)} \\
Corel5k & 0.7065(6) & 0.7133(3) & 0.7121(5) & \textbf{0.7150(1)} & 0.7044(8) & 0.7062(7) & 0.6835(9) & 0.7122(4) & 0.7145(2) \\
rcv1subset1 & 0.8926(8) & 0.9037(2) & 0.8928(7) & 0.8979(6) & 0.9022(3) & 0.9002(5) & 0.8406(9) & 0.9022(4) & \textbf{0.9096(1)} \\
rcv1subset2 & 0.8890(9) & 0.9016(4) & 0.8916(8) & 0.9006(5) & \textbf{0.9046(1)} & 0.9005(6) & 0.9001(7) & 0.9038(3) & 0.9041(2) \\
rcv1subset3 & 0.8663(8) & 0.8801(5) & 0.8821(4) & 0.8845(2) & 0.8799(6) & 0.8751(7) & 0.8605(9) & 0.8831(3) & \textbf{0.8868(1)} \\
yahoo-Art & 0.7257(8) & 0.7379(6) & 0.7424(5) & \textbf{0.7592(1)} & 0.7515(2) & 0.7251(9) & 0.7362(7) & 0.7481(3) & 0.7460(4) \\
yahoo-Business & 0.7407(9) & 0.7432(6) & 0.7450(4) & 0.7491(3) & 0.7444(5) & 0.7431(7) & 0.7410(8) & 0.7521(2) & \textbf{0.7550(1)} \\
\midrule
\textit{AveRank} & 8.11 & 5.33 & 4.56 & 3.00 & 3.78 & 6.44 & 7.56 & 3.44 & \textbf{1.67} \\\midrule
\multicolumn{10}{c} {Macro-AUCPR $\uparrow$} \\\cmidrule(l){1-10}
emotions & 0.6594(9) & 0.6706(7) & 0.6800(5) & 0.6792(6) & 0.6888(3) & 0.6876(4) & 0.6673(8) & \textbf{0.6974(1)} & 0.6928(2) \\
scene & 0.8522(9) & 0.8526(8) & 0.8543(7) & 0.8601(4) & 0.8584(5) & 0.8564(6) & 0.8614(2) & 0.8612(3) & \textbf{0.8650(1)} \\
yeast & 0.4950(7) & 0.4934(9) & 0.4953(6)& 0.5004(5)  & 0.5064(3) & 0.5051(4) & 0.4935(8) &  0.5091(2) &\textbf{0.5322(1)} \\
Corel5k & 0.1198(6) & 0.1209(5) & 0.1130(9) & 0.1224(3) & 0.1192(7) & 0.1223(4) & 0.1150(8) & 0.1226(2) & \textbf{0.1247(1)}\\
rcv1subset1 & 0.3040(8) & 0.2881(9) & 0.3105(4) & 0.3136(3) & 0.3142(2) & 0.3092(5) & 0.3047(7) & 0.3081(6) & \textbf{0.3173(1)} \\
rcv1subset2 & 0.2523(9) & 0.2747(8) & 0.3036(4) & 0.3097(2) & 0.3049(3) & 0.2996(6) & 0.2822(7) & 0.3023(5) & \textbf{0.3173(1)} \\
rcv1subset3 & 0.2360(8) & 0.2300(9) & 0.2606(2) & \textbf{0.2677(1)} & 0.2495(4) & 0.2399(6) & 0.2368(7) & 0.2432(5) & 0.2528(3) \\
yahoo-Art & 0.3444(9) & 0.3614(4) & 0.3614(5) & \textbf{0.3731(1)} & 0.3588(6) & 0.3505(8) & 0.3537(7) & 0.3655(3) & 0.3657(2) \\
yahoo-Business & 0.4206(6) & 0.4233(4) & \textbf{0.4295(1)} & 0.4259(3) & 0.4142(9) & 0.4189(7) & 0.4159(8) & 0.4229(5) & 0.4262(2) \\
\midrule
\textit{AveRank}  & 7.89 & 7.00 & 4.33 & 3.11 & 4.67 & 5.22 & 6.22 & 3.56 & \textbf{1.56} \\\midrule
\multicolumn{10}{c} {Ranking Loss $\downarrow$} \\\cmidrule(l){1-10}
emotions & 0.1927(7) & 0.1581(4) & 0.1618(6) & 0.1603(5) & 0.2014(8) & 0.1562(3) & 0.2460(9) & 0.1530(2) & \textbf{0.1515(1)} \\
scene & 0.0711(6) & 0.0718(8) & 0.0712(7) & 0.0703(5) & 0.0757(9) & 0.0685(3) & 0.0677(2) & 0.0695(4) & \textbf{0.0634(1)} \\
yeast & 0.1736(7) & 0.1839(8) & 0.1846(9) & 0.1725(6) & 0.1722(4) & 0.1702(2) & 0.1724(5) & \textbf{0.1698(1)} & 0.1712(3) \\
Corel5k & 0.2020(5) & 0.2037(7)& 0.2115(8) &  \textbf{0.1925(1)} & 0.1987(4) & 0.2023(6) & 0.2134(9) & 0.1982(3) & 0.1933(2) \\
rcv1subset1 & 0.0651(8) & 0.0596(2) & 0.0626(5) & 0.0612(3) & 0.0639(7) & 0.0629(6) & 0.0770(9) & 0.0614(4) & \textbf{0.0587(1)} \\
rcv1subset2 & 0.0672(8) & 0.0603(4) & 0.0621(7) & 0.0618(5) & \textbf{0.0596(1)} & 0.0620(6) & 0.6760(9) & 0.0602(3) & 0.0596(2) \\
rcv1subset3 & 0.0740(8) & 0.0711(6) & 0.0697(3) & 0.0680(2) & 0.0708(5) & 0.0725(7) & 0.0868(9) & 0.0701(4) & \textbf{0.0678(1)} \\
yahoo-Art & 0.1108(8) & 0.1054(6) &0.1064(7)  & 0.1006(3) & 0.1007(4) & 0.1109(9) & 0.1003(2) & 0.1009(5) & \textbf{0.0988(1)} \\
yahoo-Business & 0.0337(7) & 0.0368(9) & 0.0352(8) & 0.0304(2) & 0.0326(5) & 0.0317(4) & 0.0331(6) & 0.0304(3) & \textbf{0.0284(1)} \\
\midrule
\textit{AveRank} & 7.11 & 6.00 & 6.67 & 3.56 &5.22 & 5.11 & 6.67 & 3.22 & \textbf{1.44}\\\bottomrule
\end{tabular}
}
\label{tab:C2AE}
\end{table}



% Specifically, for multi-label datasets, it is generally observed that datasets with higher feature dimensions also tend to have higher label dimensions, and they often exhibit higher imbalance as well, such as (rcv1subset1, rcv1subset2, rcv1subset3, Corel5k), LSDMLO has significant effects on such datasets. 


% \begin{table*}[!h] 
%   \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccccccc}
% \toprule
% Metric & learner & Base & MLSMOTE\textsubscript{U} & MLSMOTE\textsubscript{R}  & MLSOL  & MLROS & MLRUS  & RHwRSMT & MLBOTE & LSDMLO \\ \midrule
% \multirow{7}{*}{Macro-F} 
% &BR & 5.11* &  6.67* & 4.89* & 3.33 & 4.78*  & 6.00* & 9.00* & 3.78*  & \textbf{1.44(7/0)} \\
% &MLkNN & 6.56* & 5.00* & 3.56 & 2.89 & 5.22* & 7.33* & 8.78* & 3.22  & \textbf{2.44(5/0)} \\
% &CC & 6.22* & 6.00* & 5.11* & 3.22  & 4.11  & 5.78*& 9.00* & 3.89  & \textbf{1.67(5/0)} \\
% &RAkEL & 6.78* & 6.11* & 5.56* & 3.56  & 3.22  & 5.78* & 9.00* & 3.78* & \textbf{1.22(6/0)} \\
% &COCOA & 6.56* & 5.56* & 4.33* & 3.56  & 3.89*  & 7.78* & 8.00* & 4.00* & \textbf{1.33(7/0)} \\
% &C2AE & 7.67* & 5.89* & 4.44* & 4.22* & 4.56* & 4.89* & 7.78* & 3.67 & \textbf{1.89(7/0)} \\
% \cmidrule(l){2-11} 
% & \textit{Ave} & 6.08 & 5.74 & 4.89 & 3.45 & 4.10 & 6.01 & 8.67 & 3.67 & \textbf{1.80} \\
% \midrule
% \multirow{7}{*}{Macro-AUC} 
% &BR & 6.44* & 4.78* & 5.78* & 2.89  & 6.78* & 7.56* & 6.22* & 3.22  & \textbf{1.33(6/0)} \\
% &MLkNN & 5.44* & 6.11* & 6.00* & 3.56  & 3.89 & 8.00* & 7.67* & 2.33  & \textbf{2.00(5/0)} \\
% &CC & 5.44* & 6.78* & 4.11* & 3.67  & 4.67* & 6.33* & 8.89* & 3.56  & \textbf{1.56(6/0)} \\
% &RAkEL & 8.00* & 5.22* & 4.56* & 3.44  & 4.22* & 7.22* & 6.78* & 3.89  & \textbf{1.67(6/0)} \\
% &COCOA & 4.78* & 6.00* & 4.67* & 3.89  & 4.22* & 7.22* & 8.56* & 4.11* & \textbf{1.56(7/0)} \\
% &C2AE & 8.11* & 5.33* & 4.56* & 3.00 & 3.78* & 6.44* & 7.56* & 3.44* & \textbf{1.67(7/0)} \\
% \cmidrule(l){2-11} 
%  &\textit{Ave}& 6.22 & 5.74 & 4.56 & 3.33 & 4.56 & 6.44 & 7.78 & 3.56 & \textbf{1.56} \\
%  \midrule
% \multirow{7}{*}{Macro-AUCPR} 
% &BR & 5.78* & 7.56* & 5.33* & 3.67* & 5.33* & 5.67* & 7.67* & 2.89  & \textbf{1.11(7/0)} \\
% &MLkNN & 6.22* & 6.00* & 4.11* & 3.22 & 4.89* & 7.22* & 7.89* & 3.56  & \textbf{1.89(6/0)} \\
% &CC & 5.78* & 7.78* & 5.56* & 3.11 & 3.78* & 6.22* & 8.00* & 3.56 & \textbf{1.22(6/0)} \\
% &RAkEL & 5.89* & 6.56* & 5.33* & 3.11 & 4.67* & 6.78* & 8.00* & 2.89  & \textbf{1.78(6/0)} \\
% &COCOA & 5.22* & 7.56* & 6.22* & 3.22 & 4.00* & 5.44* & 8.22* & 3.56 & \textbf{1.56(6/0)} \\
% &C2AE & 7.89* & 7.00* & 4.33* & 3.11 & 4.67* & 5.22* & 6.22* & 3.56* & \textbf{1.56(7/0)}\\
% \cmidrule(l){2-11} 
% & \textit{Ave}& 6.13 & 7.08 & 5.15 & 3.43 & 4.56 & 6.09 & 7.67 & 3.34 & \textbf{1.58} \\
% \midrule
% \multirow{7}{*}{Ranking Loss} 
% &BR & 6.33* & 4.78* & 6.11* & 3.56 & 5.33* & 5.89* & 7.56* & 3.67*  & \textbf{1.78(7/0)} \\
% &MLkNN & 4.56 & 6.44* & 7.00* & 5.00* & 2.56  & 3.67 & 8.00* & 5.33* & \textbf{2.44(5/0)} \\
% &CC & 4.22* & 7.22* & 5.56* & 3.44   & 5.00* & 5.44* & 9.00* & 2.78  & \textbf{2.33(6/0)} \\
% &RAkEL & 5.44* & 5.89* & 6.00* & 3.11  & 5.44* & 5.78* & 7.56* & 3.67 & \textbf{2.11(6/0)} \\
% &COCOA & 7.00* & 6.00* & 6.33* & 4.67* & 3.33 & 6.89* & 5.11* & 3.44   & \textbf{2.22(6/0)} \\
% &C2AE & 7.11* & 6.00* & 6.67* & 3.56* &5.22* & 5.11* & 6.67* & 3.22 & \textbf{1.44(7/0)} \\ 
%  \cmidrule(l){2-11} 
%  & \textit{Ave} & 5.78 & 5.93 & 6.04 & 4.04 & 4.59 & 5.46 & 7.32 & 3.74 & \textbf{2.11}\\ \bottomrule
% \end{tabular}
% }
% \caption{The average rank and statistical tests under six base learners. The parenthesis ($n_1$/$n_2$) indicates the corresponding method is significantly superior to $n_1$ methods and inferior to $n_2$ methods based on the Wilcoxon signed rank test with Bergman-Hommel's correction at the 5\% level. The best methods are highlighted by \textbf{boldface.}
% }
% \label{ta:total}
% \end{table*}

\begin{table*}[!h] 
\caption{The average rank and statistical tests under six base learners. The parenthesis ($n_1$/$n_2$) indicates the corresponding method is significantly superior to $n_1$ methods and inferior to $n_2$ methods based on the Wilcoxon signed rank test with Bergman-Hommel's correction at the 5\% level. The best methods are highlighted by \textbf{boldface.}
}
  \centering
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
Metric & Base Learner & Base & MLSMOTE\textsubscript{U} & MLSMOTE\textsubscript{R}  & MLSOL  & MLROS & MLRUS  & RHwRSMT & MLBOTE & LSDMLO \\ \midrule
\multirow{7}{*}{Macro-F} & BR & 5.11(1/1) & 6.67(1/4) & 4.89(1/1) & 3.33(2/1) & 4.78(2/1) & 6.00(1/1) & 9.00(0/8) & 3.78(2/0) & \textbf{1.44(7/0)} \\
 & MLkNN & 6.56(1/5) & 5.00(2/2) & 3.56(3/1) & 2.89(5/0) & 5.22(4/3) & 7.33(1/6) & 8.78(0/8) & 3.22(4/0) & \textbf{2.44(5/0)} \\
 & CC & 6.22(1/2) & 6.00(1/2) & 5.11(1/1) & 3.22(2/0) & 4.11(1/1) & 5.78(1/1) & 9.00(0/8) & 3.89(2/1) & \textbf{1.67(7/0)} \\
 & RAkEL & 6.78(1/4) & 6.11(1/1) & 5.56(1/1) & 3.56(2/1) & 3.22(3/0) & 5.78(1/2) & 9.00(0/8) & 3.78(1/1) & \textbf{1.22(7/0)} \\
 & COCOA & 6.56(0/3) & 5.56(1/2) & 4.33(2/1) & 3.56(4/0) & 3.89(2/0) & 7.78(0/5) & 8.00(0/6) & 4.00(3/1) & \textbf{1.33(6/0)} \\
 & C2AE & 7.67(0/4) & 5.89(0/0) & 4.44(0/0) & 4.22(1/0) & 4.56(2/1) & 4.89(0/1) & 7.78(0/3) & 3.67(2/0) & \textbf{1.89(4/0)} \\ \cline{2-11} 
 & \textit{Ave}(\textit{Total}) & 6.08(4/19) & 5.74(6/11) & 4.89(8/5) & 3.45(16/2) & 4.10(14/6) & 6.01(4/16) & 8.67(0/41) & 3.67(16/3) & \textbf{1.80(36/0)} \\ \hline
\multirow{7}{*}{ \begin{tabular}[c]{@{}c@{}}Macro \\ -AUC\end{tabular} } & BR & 6.44(0/4) & 4.78(2/1) & 5.78(0/3) & 2.89(4/0) & 6.78(0/3) & 7.56(0/4) & 6.22(0/0) & 3.22(4/0) & \textbf{1.33(5/0)} \\
 & MLkNN & 5.44(1/4) & 6.11(0/4) & 6.00(0/3) & 3.56(3/0) & 3.89(4/2) & 8.00(1/5) & 7.67(0/3) & 2.33(6/0) & \textbf{2.00(6/0)} \\
 & CC & 5.44(1/1) & 6.78(1/5) & 4.11(2/1) & 3.67(2/0) & 4.67(2/2) & 6.33(1/1) & 8.89(0/8) & 3.56(3/1) & \textbf{1.56(7/0)} \\
 & RAkEL & 8.00(0/5) & 5.22(1/1) & 4.56(2/1) & 3.44(0/0) & 4.22(1/0) & 7.22(0/2) & 6.78(0/1) & 3.89(1/1) & \textbf{1.67(6/0)} \\
 & COCOA & 4.78(2/1) & 6.00(0/1) & 4.67(1/1) & 3.89(2/0) & 4.22(2/1) & 7.22(1/5) & 8.56(0/7) & 4.11(2/1) & \textbf{1.56(7/0)} \\
 & C2AE & 8.11(0/7) & 5.33(1/1) & 4.56(2/2) & 3.00(2/1) & 3.78(3/0) & 6.44(1/3) & 7.56(0/4) & 3.44(4/0) & \textbf{1.67(6/0)} \\ \cline{2-11} 
 & \textit{Ave}(\textit{Total}) & 6.22(4/22) & 5.74(5/13) & 4.56(7/10) & 3.33(13/1) & 4.56(12/8) & 6.44(4/20) & 7.78(0/23) & 3.56(20/3) & \textbf{1.56(37/0)} \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Macro \\ -AUCPR\end{tabular} } & BR & 5.78(0/1) & 7.56(0/3) & 5.33(0/1) & 3.67(1/1) & 5.33(0/3) & 5.67(0/1) & 7.67(0/2) & 2.89(3/0) & \textbf{1.11(7/0)} \\
 & MLkNN & 6.22(0/1) & 6.00(0/2)& 4.11(0/2) & 3.22(2/0) & 4.89(3/0) & 7.22(2/1) & 7.89(0/5) & 3.56(3/1) & \textbf{1.89(6/0)} \\
 & CC & 5.78(2/4) & 7.78(0/7) & 5.56(2/4) & 3.11(5/0) & 3.78(5/0) & 6.22(2/4) & 8.00(0/7) & 3.56(5/1) & \textbf{1.22(6/0)} \\
 & RAkEL & 5.89(0/2) & 6.56(1/2)& 5.33(0/3) & 3.11(3/0) & 4.67(1/2) & 6.78(0/4) & 8.00(0/3) & 2.89(5/1) & \textbf{1.78(6/0)} \\
 & COCOA & 5.22(0/1) & 7.56(0/4) & 6.22(1/4) & 3.22(3/0) & 4.00(3/0) & 5.44(0/1) & 8.22(0/5) & 3.56(3/0) & \textbf{1.56(5/0)} \\
 & C2AE & 7.89(0/4) & 7.00(0/3) & 4.33(0/0) & 3.11(3/0) & 4.67(0/1) & 5.22(1/2) & 6.22(0/3) & 3.56(4/0) & \textbf{1.56(5/0)} \\ \cline{2-11} 
 & \textit{Ave}(\textit{Total}) & 6.13(2/13) & 7.08(1/21) & 5.15(0/23) & 3.43(17/1) & 4.56(12/6) & 6.09(5/13) & 7.67(0/25) & 3.34(23/3) & \textbf{1.58(35/0)} \\ \hline
\multirow{7}{*}{ \begin{tabular}[c]{@{}c@{}}Ranking \\ Loss\end{tabular}  } & BR & 6.33(0/1) & 4.78(0/1) & 6.11(0/2) & 3.56(0/0) & 5.33(0/1) & 5.89(1/0) & 7.56(0/1) & 3.67(1/1) & \textbf{1.78(4/0)} \\
 & MLkNN & 4.56(1/0) & 6.44(0/0) & 7.00(0/3) & 5.00(0/0) & 2.56(2/0) & 3.67(2/0) & 8.00(0/5) & 5.33(1/0) & \textbf{2.44(2/0)} \\
 & CC & 4.22(2/0) & 7.22(1/5) & 5.56(1/1) & 3.44(1/0) & 5.00(2/0) & 5.44(2/2) & 9.00(0/8) & 2.78(3/0) & \textbf{2.33(4/0)} \\
 & RAkEL & 5.44(0/2) & 5.89(0/2) & 6.00(1/1) & 3.11(4/0) & 5.44(0/0) & 5.78(0/2) & 7.56(0/3) & 3.67(0/0) & \textbf{2.11(5/0)} \\
 & COCOA & 7.00(0/1) & 6.00(0/0) & 6.33(0/1) & 4.67(0/0) & 3.33(0/0) & 6.89(0/1) & 5.11(0/0) & 3.44(1/0) & \textbf{2.22(2/0)} \\
 & C2AE & 7.11(0/4) & 6.00(0/0) & 6.67(0/0) & 3.56(1/0) & 5.22(2/1) & 5.11(0/1) & 6.67(0/3) & 3.22(2/0) & \textbf{1.44(4/0)} \\ \cline{2-11} 
 & \textit{Ave}(\textit{Total}) & 5.78(3/8) & 5.93(1/8) & 6.04(2/8) & 4.04(6/0) & 4.59(6/2) & 5.46(5/6) & 7.32(0/20) & 3.74(8/0) & \textbf{2.11(21/0)} \\  \bottomrule
\end{tabular}
}
\label{ta:total}
\end{table*}



